Piecewise Polyhedral Formulations for a Multilinear Term

In this paper, we present a mixed-integer linear programming (MILP) formulation of a piecewise, polyhedral relaxation (PPR) of a multilinear term using its convex hull representation. Based on the solution of the PPR, we also present a MILP formulation whose solutions are feasible for nonconvex, multilinear equations. We then present computational results showing the effectiveness of proposed formulations on instances of standard benchmarks of nonlinear programs (NLPs) with multilinear terms and compare the proposed formulation with a traditional formulation that is built by recursively relaxing bilinear groupings of multilinear terms.

==> relaxation_tikz.tex <==
    \begin{tikzpicture}[scale=0.8]
\pgfplotsset{
    scale only axis,
    every axis/.append style = {thick},tick style = {thick,black},
}

\begin{axis}[
  axis y line*=left,
  ymin=-10, ymax=80,
  xlabel={Number of partitions},
  ylabel={Piecewise relaxation obj. value (upper bound)},
  legend style={at={(1.3,0.83)},anchor=west,draw=none},
  legend cell align={left},
  title={},
  grid
]
%
\addlegendimage{empty legend}
\addlegendentry{\hspace{-.7cm}{Upper bound}}
\addplot[very thick,red,dashed]% mark=square*, mark size=1]
  coordinates{
    (2,19.5483)
    (3,8.2407)
    (4,5.43)
    (5,5.2356)
    (6,4.6443)
    (7,3.9346)
    (8,3.6075)
    (9,3.6183)
}; \label{1234}
\addlegendentry{~$x_1 x_2 x_3 x_4$}
%
\addplot[very thick, black!30!green,dashed] % mark=square*, mark options=solid, mark size=1]
  coordinates{
    (2,31.6041)
    (3,15.4579)
    (4,11.2125)
    (5,9.7084)
    (6,7.9262)
    (7,6.9343)
    (8,6.2866)
    (9,5.9802)
}; \label{1-23-4}
\addlegendentry{~$\langle x_1 \langle x_2 x_3 \rangle \rangle \,x_4$}
%
\addplot[very thick, blue,dashed]% mark=square*, mark options=solid, mark size=1]
  coordinates{
    (2,29.0947)
    (3,14.6087)
    (4,10.6346)
    (5,9.0259)
    (6,7.5177)
    (7,6.7286)
    (8,6.1790)
    (9,5.8450)
}; \label{12-3-4}
\addlegendentry{~$\langle \langle x_1 x_2 \rangle\, x_3 \rangle\, x_4$}
%
\addplot[very thick, black,dashed] %, mark=square*, mark options=solid, mark size=1]
  coordinates{
    (2,73.9803)
    (3,51.7863)
    (4,44.6842)
    (5,44.3883)
    (6,42.7275)
    (7,41.9223)
    (8,40.6893)
    (9,40.6893)
}; \label{12-34}
\addlegendentry{~$\langle x_1 x_2 \rangle \,\langle x_3 x_4 \rangle $}
\end{axis}

\begin{axis}[
  axis y line*=right,
  ymin=-500, ymax=5000,
  xlabel={Number of partitions},
  ylabel={Computation time (sec)},
  legend style={at={(1.3,0.43)},anchor=west,draw=none},
  legend cell align={left}
]
\addlegendimage{empty legend}
\addlegendentry{\hspace{-.7cm}{Time}}
%
\addplot[only marks, red, mark=triangle*, mark size=3]
  coordinates{
    (2,0.05)
    (3,0.29)
    (4,1.44)
    (5,8.6)
    (6,50.31)
    (7,288.47)
    (8,1260.77)
    (9,3256.23)
}; \label{1234-t}
\addlegendentry{~$x_1 x_2 x_3 x_4$}
%
\addplot[only marks, black!30!green, mark=triangle*, mark size=3]
  coordinates{
    (2,0.03)
    (3,0.2)
    (4,1.25)
    (5,3.84)
    (6,17.94)
    (7,54.6)
    (8,91.62)
    (9,241.6)
}; \label{1-23-4-t}
\addlegendentry{~$\langle x_1 \langle x_2 x_3 \rangle \rangle\, x_4$}
%
\addplot[only marks, blue, mark=triangle*, mark size=3]
  coordinates{
    (2,0.04)
    (3,0.14)
    (4,0.64)
    (5,2.41)
    (6,7.77)
    (7,21.21)
    (8,55.2)
    (9,129.71)
}; \label{12-3-4-t}
\addlegendentry{~$\langle \langle x_1 x_2 \rangle \,x_3 \rangle\, x_4$}
%
\addplot[only marks, black, mark=triangle*, mark size=3]
  coordinates{
    (2,0.03)
    (3,0.06)
    (4,0.2)
    (5,0.24)
    (6,0.37)
    (7,0.67)
    (8,2.21)
    (9,3.21)
}; \label{12-34-t}
\addlegendentry{~$\langle x_1 x_2 \rangle \,\langle x_3 x_4 \rangle $}
\end{axis}

\end{tikzpicture}
